Learning with Noise: Enhance Distantly Supervised Relation Extraction with Dynamic Transition Matrix

Distant supervision significantly reduces human efforts in building training data for many classification tasks. While promising, this technique often introduces noise to the generated training data, which can severely affect the model performance. In this paper, we take a deep look at the application of distant supervision in relation extraction. We show that the dynamic transition matrix can effectively characterize the noise in the training data built by distant supervision. The transition matrix can be effectively trained using a novel curriculum learning based method without any direct supervision about the noise. We thoroughly evaluate our approach under a wide range of extraction scenarios. Experimental results show that our approach consistently improves the extraction results and outperforms the state-of-the-art in various evaluation scenarios.

==> motivation.tex <==
\section{Motivation}
\todo{ZW: We need a concrete example here to demonstrate what kind of noise can exist in the data and their impact on relation extraction. We then use this example to explain our approach.}
\blue{F: this could be put into the introduction, saying different types of noises in the data, and all thoses noises can be modeled by TM. }

As a motivation example, consider xx...

This example shows that noisy data can have a significant impact on relation extraction. What we like to have is a technique that can xxx.
In the remainder of this paper, we describe such an approach based on xxx. 
